AutoSketch: VLM-assisted Style-Aware Vector Sketch Completion

The ability to automatically complete a partial sketch that depicts a complex scene, e.g., "a woman chatting with a man in the park", is very useful. However, existing sketch generation methods create sketches from scratch; they do not complete a partial sketch in the style of the original. To address this challenge, we introduce AutoSketch, a styleaware vector sketch completion method that accommodates diverse sketch styles. Our key observation is that the style descriptions of a sketch in natural language preserve the style during automatic sketch completion. Thus, we use a pretrained vision-language model (VLM) to describe the styles of the partial sketches in natural language and replicate these styles using newly generated strokes. We initially optimize the strokes to match an input prompt augmented by style descriptions extracted from the VLM. Such descriptions allow the method to establish a diffusion prior in close alignment with that of the partial sketch. Next, we utilize the VLM to generate an executable style adjustment code that adjusts the strokes to conform to the desired style. We compare our method with existing methods across various sketch styles and prompts, performed extensive ablation studies and qualitative and quantitative evaluations, and demonstrate that AutoSketch can support various sketch scenarios.

==> conf_preamble.tex <==
\RequirePackage{ifthen}
\newcommand{\conf}{siggraph}
% submit, camera, final....
\newcommand{\stage}{submit}
% \newcommand{\track}{journal}
% \newcommand{\mode}{main}
% \def\conf{cvpr}
% \input{siggraph_preamble}
\newcommand{\isequal}[3]{
    \ifthenelse{\equal{#1}{#2}}{
        #3
    }{}    
}

% \isequal{\conf}{siggraph}{
% \ifthenelse{\equal{\mode}{main}}{
%         \input{siggraph/siggraph_preamble}
%     }
%     {
%         \input{siggraph/siggraph_supp_preamble}
%     }
% }


\isequal{\conf}{siggraph}{\input{siggraph/siggraph_preamble}}
% \isequal{\conf}{cvpr}{\input{cvpr/cvpr_preamble}}
% \isequal{\conf}{eccv}{\input{eccv/eccv_preamble}}
% \isequal{\conf}{uist}{\input{uist/uist_preamble}}
% \isequal{\conf}{chi}{\input{chi/chi_preamble}}
% \isequal{\conf}{pg}{\input{cgf/cgf_preamble}}
% \isequal{\conf}{tvcg}{\input{ieeetrans/ieeetrans_preamble}}
% \isequal{\conf}{neurips}{\input{neurips/neurips_preamble}
% \input{neurips/neurips_metadata}}
% \isequal{\conf}{iclr}{\input{iclr/iclr_preamble}}


% \ifthenelse{\equal{\conf}{siggraph}}{
%     \input{siggraph/siggraph_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{cvpr}}{
%     \input{cvpr/cvpr_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{eccv}}{
%     \input{eccv/eccv_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{uist}}{
%     \input{uist/uist_preamble}
% }
% {
% }

==> fig_files/code_adjust_ablation_fig.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/code_adjust_ablation_v1.pdf}
  \caption{
\textbf{Style adjustment code ablation study example.}
Many important strokes depicted in (a) the style-agnostic completed sketch are missing from (b) the VLM direct editing results. 
In contrast, (c) our method effectively preserves such strokes while adjusting the styles. 
}
  \label{fig:code_ablation}
\end{figure}

==> fig_files/diff_prompt_sketch_fig.tex <==
\begin{figure}[!h]
  \centering
  \includegraphics[width=\linewidth]{figs/diff_prompt_sketch_v0.pdf}
  \caption{
\textbf{Various sketch scenarios.}
(a) Given the same prompt, our method can generate completed sketches that depict the same content in different styles that align with those of the user-provided partial sketches. 
(b) Given the same partial sketch, our method can generate different completed sketches representing the contents of various prompts.
}
  \label{fig:diff_promp_sketch}
\end{figure}

==> fig_files/iter_edits_fig.tex <==
\begin{figure*}[!h]
  \centering
  \includegraphics[width=\linewidth]{figs/iter_edit_examples.pdf}
  \caption{
\textbf{Examples of iterative sketch completion.}
% Given the same partial sketch, our method enables use
% \todo{Think about can we include a comparison with SketchDreamer here?}
After the initial sketch completion, the user can keep the strokes generated in the first completion and (a) edit the sketch or (b) update the input prompt .
Then, our method will complete the sketch once again to add more details.
(The blue and green line denotes the input partial sketch of the first and second iteration, respectively.)
}
\label{fig:iter_edit}
\end{figure*}

==> fig_files/limitation_fig.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/limitation.pdf}
  \caption{
  % \todo{Complete caption.}
\textbf{Limitation.} 
Our method cannot generate completed sketch that accurately depict content in the input prompt and maintain the styles in the partial sketch with (a) a broken guidance image generated by the ControlNet or (b) a broken style adjustment code generated by the VLM.
}
  \label{fig:limitation}
\end{figure}

==> fig_files/manual_comparison_fig.tex <==
\begin{figure}[!h]
  \centering
  \includegraphics[width=\linewidth]{figs/manual_comparison.pdf}
  \caption{
  % \todo{Complete the caption after we collected user evaluation results.}
\textbf{Comparison with manual sketch completion.}
}
  \label{fig:manual_comparison}
\end{figure}

==> fig_files/prompt_stylization_ablation_fig.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/prompt_stylization_ablation_v1.pdf}
  \caption{
\textbf{Prompt stylization ablation study example.} 
(a) The guidance image generated using the partial sketch and the original input prompt, which lacks style descriptions, does not align with the style of the partial sketch. 
Thus, our method could not then generate a final completed sketch that accurately depicted the complete content and the desired style.
(b) In contrast, use of a stylized prompt created a guidance image that was consistent with the style, leading to a more completed sketch.
(The \textbf{bold text} in the prompt are style descriptions generated by the VLM.)
}
\label{fig:prompt_stylization_ablation}
\end{figure}

==> fig_files/same_prompt_result_fig.tex <==
\begin{figure}[!h]
  \centering
  \includegraphics[width=\linewidth]{figs/same_prompt_cases_v0.pdf}
  \caption{
\todo{Revise the caption...}
\textbf{Same prompt cases.} blahblahblah...
}
  \label{fig:same_prompt_fig}
\end{figure}

==> fig_files/stylized_prompt_example_fig.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/stylized_prompt.pdf}
  \caption{
\ichao{ignore.}\textbf{Prompt stylization examples.} blahblahblah...
}
  \label{fig:stylized_prompt}
\end{figure}

==> fig_files/vlm_ablation_fig.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figs/vlm_ablation_v0.pdf}
  \caption{
\textbf{VLM generalization example.} 
Our method utilizing (a) GPT-4o and (b) Gemini as the VLM can generate completed sketches that exhibit similar content and style based on the provided partial sketch.
}
  \label{fig:vlm_ablation}
\end{figure}
